All the Massive Galaxy Overdensities during Reionization: JWST Rest-Frame Optical Selection Reveals Young, Chemically Evolved Galaxies Embedded in Dense, Neutral Gas at z > 5

The high-redshift progenitors of present-day galaxy clusters are believed to substantially contribute to the global star-formation rate density and drive the large-scale reionization of the Universe. Here we present a blind and unbiased search for and characterization of galaxy overdensities during the reionization epoch at redshifts $z\sim 5.5-7$, based on rest-frame optical JWST/NIRCam grism spectroscopy of the Abell\,2744 lensing field as part of the JWST-ALT survey. Using a physically-motivated, cosmological inference Friends-of-Friends (FoF) algorithm, we identify six galaxy overdensities, including five robust systems at $z=5.66$ to $6.77$. They are all characterized by total halo masses $M_{\rm halo} \gtrsim 10^{11}\,M_{\odot}$ inferred from a range of proxies. We find that the galaxy members in these overdense environments are on average less massive though equally metal-rich, and generally comprised of younger stellar populations as indicated from their bluer spectral slopes less prominent Balmer breaks, than field galaxies at similar redshifts. Further, we use this novel rest-frame optical selection of galaxy proto-clusters to infer the fraction and 3D distribution of strong Lyman-$\alpha$ emitters (LAEs) and damped Lyman-$\alpha$ absorbers (DLAs) in the overdensity environments. We find that two out of six galaxy overdensities have excess \hi\ absorption compared to the field-average, while the other four are consistent within their large scatter in density. These results present the first direct observational constraints on the tomography of the dense, neutral gas reservoirs in large-scale galaxy overdensities at $z>5$ and highlight the limitations of pre-JWST searches for reionization-era galaxy overdensities relying on the detection of strong LAEs alone.[Abridged]

==> authors.tex <==
Chamilla Terp
Kasper E. Heintz
Jorrytt Matthee
Rohan P. Naidu
Pascal A. Oesch
Alberto Torralba

Callum Witten
